An epistemic approach to model uncertainty in data-graphs

Graph databases are becoming widely successful as data models that allow to effectively represent and process complex relationships among various types of data. As with any other type of data repository, graph databases may suffer from errors and discrepancies with respect to the real-world data they intend to represent. In this work we explore the notion of probabilistic unclean graph databases, previously proposed for relational databases, in order to capture the idea that the observed (unclean) graph database is actually the noisy version of a clean one that correctly models the world but that we know partially. As the factors that may be involved in the observation can be many, e.g, all different types of clerical errors or unintended transformations of the data, we assume a probabilistic model that describes the distribution over all possible ways in which the clean (uncertain) database could have been polluted. Based on this model we define two computational problems: data cleaning and probabilistic query answering and study for both of them their corresponding complexity when considering that the transformation of the database can be caused by either removing (subset) or adding (superset) nodes and edges.

==> demos/teo-subset-no-fijo.tex <==
\begin{theorem}
\label{teo:subsetNpComplete} %\label{teo-subset-fixed}
The problem \decisionProblem{data cleaning lower bound} is \textsc{NP-complete}, even when considering Subset PUGDs with no node deletions (i.e. $\aRealizationModel(G)(G') > 0$ implies $V_\aGraph = V_\aGraph'$) and a $\Sigma$-uniform $\aRealizationModel$ such that $\aInverseRealizationModel_{\aProbabilisticDatabase, \aRealizationModel}$ is efficiently computable.
\end{theorem}

\begin{proof}
The problem is in \textsc{NP}: when given a certificate data-graph $I$ it suffices to check that  $\aInverseRealizationModel(\aGraph')(I) > b$. This last inequality can be checked in $poly(|I|+|\aGraph'|)$ by definition of $\aInverseRealizationModel$, and given the restrictions on $\aRealizationModel$ of not allowing node deletions we know that any valid certificate will satisfy $|I| = \bigO{poly(|\aGraph'|})$.\footnote{This observation remains valid if $\aRealizationModel$ is conditioned to assign probability 0 to transitions between data-graphs $\aGraph'$ and $\aGraph''$ whose size differ exponentially. As was argued in the definitions, this is a reasonable practical restriction}   

For the hardness, let us reduce \decisionProblem{SAT} to the problem of \decisionProblem{data cleaning lower bound} with $|\Sigma_e|>1$ and a $\Sigma$-uniform $\aRealizationModel$. Given a formula $\aFormula$ of $n$ variables $x_1\ldots x_n$ (that can be evaluated in $poly(|\aFormula|)$ given the $n$ assignments of its variables) we will define a PUGD $\aPUGD = (\aProbabilisticDatabase,\aRealizationModel,\aGraph')$ and a bound $b$ such that $\aFormula$ is satisfiable if and only if there exists a data-graph $I_m$ such that $\aInverseRealizationModel(\aGraph')(I_m) > b$. The PUGD $\aPUGD$ and the bound $b$ will be computable in $poly(|\aFormula|)$ time.

For this proof, consider $\{e_1,e_2\} \subseteq \Sigma_e$ and $\{c\} \subseteq \Sigma_n$. That is, we prove the hardness of the problem only when there are at least two different edge labels.

We define $\aGraph'$ as the data-graph with $n+2$ nodes with data value $c$ and no edges: $\aGraph' = (\{v_i$ $|$ $1\leq i \leq n\} \cup \{\top, null\}, L, D)$ where $L(w,z) = \emptyset$ and $D(w) = c$ $\forall w, z \in V_{\aGraph'}$. 

The function $\aProbabilisticDatabase$ is defined in the following way:

\[ \mathcal{I}(I) = \begin{cases} 
     \frac{1+\eval{I}}{2^{n+1}} & \text{if }\valid{e_1} \\
      \frac{1-\eval{I}}{2^{n+1}} & \text{if }\valid{e_2} \\
      0 & \text{otherwise}.

   \end{cases}
\]

The predicate $\valid{e}$ is true when $V_I = V_{\aGraph'}$, there is an edge $(\top,e,null)$ and all the rest of the edges are of the form $(v_i,e,\top)$ for some $1\leq i\leq n$. The expression $\eval{I}$ evaluates to 1 if the formula $\aFormula$ is satisfied by the assignment to the variables $x_i$ defined through the graph $I$, and to 0 otherwise. The variable $x_i$ is set as $\top$ if $(v_i,e,\top) \in E_I$ for some $e \in \{e_1,e_2\}$. Note that $\aProbabilisticDatabase$ is a probabilistic database:
\begin{align*}
\sum_{I \in \aProbabilisticDatabase} \aProbabilisticDatabase(I) &= 
\sum_{e \in \{e_1,e_2\}} \sum_{I : \valid{e}} \aProbabilisticDatabase(I) =
\sum_{I:\valid{e_1}} \left(\frac{1+\eval{I}}{2^{n+1}} + \frac{1-\eval{I}}{2^{n+1}} \right) 
    \\
&=\sum_{I:\valid{e_1}} \frac{2}{2^{n+1}} = 2^n \frac{1}{2^n} = 1.
\end{align*}

The second equality follows because there is a data-graph $I$ that satisfies $\valid{e_1}$ if and only if there exists a data-graph $I'$ that satisfies $\valid[I']{e_2}$. More precisely, the edges of these two data-graphs coincide except for the edge labels (that is, they have the same `topology' if we ignore the labels of the edges) and so there is a bijection between the set of data-graphs that satisfy $\valid{e_1}$ and $\valid{e_2}$, and these sets are disjoint.\footnote{Observe that if we do not include the edge between $\top$ and $null$ this sets would not be disjoint because of the data-graph $I = \aGraph'$, which would map into itself through the function that changes edge labels.}

We now define $b = \frac{1}{2^{n+1}}$ and $\aRealizationModel(I)(\aGraph') = 1$ for every data-graph $I$. Notice that this $\aRealizationModel$ is $\Sigma$-uniform, and that $\aInverseRealizationModel_{\aProbabilisticDatabase, \aRealizationModel}(\aGraph')(I)$ can be computed efficiently. This follows since:
$$
\aInverseRealizationModel_{\aProbabilisticDatabase, \aRealizationModel}(\aGraph')(I) = \frac{\aProbabilisticDatabase(I) \times \aRealizationModel(I)(\aGraph')}{\sum \aProbabilisticDatabase(I') \times \aRealizationModel(I')(\aGraph')} = \frac{\aProbabilisticDatabase(I)}{\sum \aProbabilisticDatabase(I')} = \aProbabilisticDatabase(I)
$$

Next, we prove that $\aFormula$ is satisfiable if and only if there exists a graph $I \in \aProbabilisticDatabase$ such that $\aInverseRealizationModel(\aGraph')(I) > b$.

$\implies$) Let $\nu:var(\aFormula) \to \{\top,\bot\}$ be a valuation over the variables of $\aFormula$ that satisfies $\aFormula$. 
We define the data-graph $I = (\{v_i$ $|$ $1\leq i \leq n\} \cup \{\top\}, L, D)$ where if $\nu(x_i) = \top$, then $D(v_i)=c$ and $L(v_i,\top) = \{e_1\}$ for each $i=1, \ldots, n$. 
Otherwise, $L(w,z) = \emptyset$ for every pair $w,z \in V_I$. 
It follows from the previous discussion that $\aInverseRealizationModel(\aGraph')(I) = \frac{1+1}{2^{n+1}} \times 1 = \frac{1}{2^n} > \frac{1}{2^{n+1}} = b$.

$\impliedby$) Let $I$ be a data-graph $I \in \aProbabilisticDatabase$ that satisfies $\aInverseRealizationModel(\aGraph')(I) > \frac{1}{2^{n+1}}$. Hence, every edge label of $I$ must be $e_1$. We can define a valuation $\nu$ over $var(\aFormula)$ based on $I$ as: 
$$\nu(x_i) = \top \iff L(v_i,\top) = \{e_1\}$$ 
for $1\leq i \leq n$. Since $I$ satisfies $\eval{I}$ (otherwise it is not possible that $\aInverseRealizationModel(\aGraph')(\aProbabilisticDatabase) > b$), we know that $\nu$ satisfies $\aFormula$.
\end{proof}

Observe that in this construction both $\aProbabilisticDatabase$ and $\aRealizationModel$ depend strongly on the observed unclean data-graph $\aGraph'$. It makes sense to assume that $\aProbabilisticDatabase$ and $\aRealizationModel$ are both \textit{fixed}, and \textit{independent} of the observed state of the database, since they may represent some gained knowledge around the expected structure of the data. \widesanti{Acá estaría bueno que linkeemos alguna parte del trabajo donde trabajemos con $I$ y $R$ fijo. Ver si sale la demo sin fijar $\aProbabilisticDatabase$ y $\aRealizationModel$, usando el mundo de grafos "que representan fórmulas con su asignación"}


==> demos/teo-superset-no-fijo.tex <==
Since node additions are not allowed, the preimage of an observed graph $\aGraph$ through $\aRealizationModel$ has to be a subset of the graphs built with the same set of nodes from $\aGraph'$ and a subset of its edges. Therefore, we can ask for the data-graph $I_m$ with $\aInverseRealizationModel(G')(I_m) > b$ as a witness. 

For the hardness, as in the subset case, we will reduce 3-SAT to the Superset PUGD data cleaning problem under the stated conditions. Given a 3-SAT formula $\phi$ of $n$ variables and $m$ clauses we define the PUGD $\aPUGD = (\aProbabilisticDatabase, \aRealizationModel, (V,L,D))$ and the bound $b$ in the following way:
\begin{align*}
& V  = \{x_i : 1 \leq i \leq n\} \cup \{\top,null\}\\
& L(x_i,\top)  = \{e_1,e_2\} \text{ for } 1\leq i \leq n \\
& L(v,w)  = \emptyset \text{ for any other case } \\
& D(v)  = c \text{ for any } v \in V \\
& \aRealizationModel(I)(\aGraph') = 1 \text{ for any } I \subseteq \aGraph \\
& b = \frac{1}{2^{n+1}} 
\end{align*}


Finally, the function $\aProbabilisticDatabase$ is defined as in Theorem~\ref{teo:subsetNpComplete} as:

\[ \mathcal{I}(I) = \begin{cases} 
     \frac{1+\eval{I}}{2^{n+1}} & \text{if }\valid{e_1} \\
      \frac{1-\eval{I}}{2^{n+1}} & \text{if }\valid{e_2} \\
      0 & \text{otherwise}.

   \end{cases}
\]

%in the same way as in the proof of the subset-PUGD case.

It follows analogously as in the Subset PUGD case that any graph $I$ that satisfies $\aInverseRealizationModel(\aGraph')(I) > b$ encodes an assignment of the $n$ variables from $\phi$ that satisfies the formula (and vice versa). Also note that the construction of $\aPUGD$ and $b$ can be done in time $poly(n)$.
